What Can We Learn from Unlearnable Datasets?

In an era of widespread web scraping, unlearnable dataset methods have the potential to protect data privacy by preventing deep neural networks from generalizing. But in addition to a number of practical limitations that make their use unlikely, we make a number of findings that call into question their ability to safeguard data. First, it is widely believed that neural networks trained on unlearnable datasets only learn shortcuts, simpler rules that are not useful for generalization. In contrast, we find that networks actually can learn useful features that can be reweighed for high test performance, suggesting that image protection is not assured. Unlearnable datasets are also believed to induce learning shortcuts through linear separability of added perturbations. We provide a counterexample, demonstrating that linear separability of perturbations is not a necessary condition. To emphasize why linearly separable perturbations should not be relied upon, we propose an orthogonal projection attack which allows learning from unlearnable datasets published in ICML 2021 and ICLR 2023. Our proposed attack is significantly less complex than recently proposed techniques.

==> figures/data/cw-unlearnable.tex <==
\addplot[violet]
coordinates { % Test Acc
(0, 13.530)
(1, 13.070)
(2, 11.700)
(3, 14.810)
(4, 17.340)
(5, 13.020)
(6, 11.630)
(7, 12.700)
(8, 11.180)
(9, 11.390)
(10, 13.210)
(11, 16.050)
(12, 11.180)
(13, 10.610)
(14, 14.900)
(15, 13.450)
(16, 11.810)
(17, 13.770)
(18, 15.270)
(19, 14.490)
(20, 15.350)
(21, 15.160)
(22, 17.090)
(23, 15.040)
(24, 15.610)
(25, 15.830)
(26, 16.630)
(27, 15.610)
(28, 16.300)
(29, 15.680)
(30, 14.180)
(31, 13.840)
(32, 12.710)
(33, 14.180)
(34, 14.420)
(35, 13.380)
(36, 13.610)
(37, 10.850)
(38, 12.810)
(39, 13.090)
(40, 12.430)
(41, 11.860)
(42, 12.230)
(43, 16.510)
(44, 11.140)
(45, 12.040)
(46, 11.640)
(47, 11.590)
(48, 12.200)
(49, 11.290)
(50, 11.310)
(51, 11.300)
(52, 11.270)
(53, 10.860)
(54, 11.330)
(55, 11.420)
(56, 11.320)
(57, 11.490)
(58, 11.630)
(59, 11.280)
};
    


==> figures/data/cwrandom.tex <==
\addplot[violet]
coordinates { % Test Acc
(0, 42.650)
(1, 54.570)
(2, 60.430)
(3, 58.170)
(4, 10.730)
(5, 10.270)
(6, 11.190)
(7, 10.080)
(8, 10.010)
(9, 10.100)
(10, 10.800)
(11, 10.000)
(12, 10.000)
(13, 9.910)
(14, 10.060)
(15, 12.560)
(16, 10.000)
(17, 10.000)
(18, 9.930)
(19, 9.740)
(20, 12.520)
(21, 10.460)
(22, 10.930)
(23, 12.490)
(24, 10.250)
(25, 9.910)
(26, 9.980)
(27, 9.520)
(28, 13.000)
(29, 8.890)
(30, 10.090)
(31, 9.880)
(32, 9.660)
(33, 11.320)
(34, 10.040)
(35, 10.090)
(36, 10.740)
(37, 12.040)
(38, 10.540)
(39, 10.890)
(40, 8.570)
(41, 9.980)
(42, 10.290)
(43, 9.020)
(44, 8.150)
(45, 10.590)
(46, 10.920)
(47, 9.920)
(48, 10.050)
(49, 10.510)
(50, 10.750)
(51, 10.660)
(52, 10.810)
(53, 10.780)
(54, 11.630)
(55, 11.420)
(56, 11.400)
(57, 10.990)
(58, 11.350)
(59, 11.350)
};
    


==> figures/data/dfr-cw-unlearnable.tex <==
\addplot[violet, densely dashed]
coordinates { % Fine-tune
(0, 26.670)
(1, 26.710)
(2, 25.410)
(3, 26.760)
(4, 26.040)
(5, 27.010)
(6, 26.890)
(7, 28.240)
(8, 25.300)
(9, 26.620)
(10, 25.660)
(11, 28.830)
(12, 26.040)
(13, 23.560)
(14, 25.380)
(15, 24.500)
(16, 24.120)
(17, 24.160)
(18, 24.950)
(19, 27.610)
(20, 24.140)
(21, 26.000)
(22, 26.360)
(23, 25.890)
(24, 26.670)
(25, 25.550)
(26, 26.000)
(27, 10.000)
(28, 27.370)
(29, 24.860)
(30, 22.500)
(31, 26.660)
(32, 25.740)
(33, 23.600)
(34, 23.460)
(35, 27.090)
(36, 23.330)
(37, 22.230)
(38, 25.190)
(39, 24.540)
(40, 24.920)
(41, 21.950)
(42, 23.590)
(43, 25.990)
(44, 10.000)
(45, 21.410)
(46, 22.360)
(47, 23.850)
(48, 20.880)
(49, 21.520)
(50, 22.690)
(51, 24.040)
(52, 22.250)
(53, 23.480)
(54, 21.710)
(55, 20.850)
(56, 21.400)
(57, 23.430)
(58, 22.270)
(59, 22.700)
};

==> figures/data/dfr-cwrandom.tex <==
\addplot[violet, densely dashed]
coordinates { % Fine-tune
(0, 46.890)
(1, 57.250)
(2, 64.470)
(3, 66.790)
(4, 47.970)
(5, 44.290)
(6, 41.080)
(7, 41.340)
(8, 39.320)
(9, 37.070)
(10, 32.260)
(11, 30.700)
(12, 29.640)
(13, 30.500)
(14, 29.810)
(15, 31.500)
(16, 29.360)
(17, 26.720)
(18, 29.160)
(19, 28.580)
(20, 27.180)
(21, 28.540)
(22, 26.340)
(23, 23.990)
(24, 23.710)
(25, 25.850)
(26, 21.400)
(27, 22.400)
(28, 22.800)
(29, 20.030)
(30, 22.900)
(31, 22.510)
(32, 21.340)
(33, 23.530)
(34, 23.470)
(35, 22.640)
(36, 21.910)
(37, 20.930)
(38, 19.910)
(39, 21.410)
(40, 19.210)
(41, 20.770)
(42, 20.920)
(43, 20.450)
(44, 18.580)
(45, 18.560)
(46, 20.220)
(47, 19.090)
(48, 19.800)
(49, 19.520)
(50, 19.820)
(51, 19.660)
(52, 19.430)
(53, 19.550)
(54, 19.650)
(55, 18.380)
(56, 18.990)
(57, 18.840)
(58, 18.330)
(59, 19.120)
};

==> figures/data/dfr-error-max.tex <==
\addplot[violet, densely dashed]
coordinates { % Fine-tune
(0, 49.080)
(1, 58.390)
(2, 58.250)
(3, 58.300)
(4, 60.240)
(5, 60.280)
(6, 59.930)
(7, 61.340)
(8, 62.270)
(9, 62.810)
(10, 64.350)
(11, 63.720)
(12, 63.120)
(13, 62.330)
(14, 59.340)
(15, 62.240)
(16, 63.870)
(17, 63.900)
(18, 63.850)
(19, 63.860)
(20, 61.700)
(21, 65.400)
(22, 63.740)
(23, 59.920)
(24, 63.140)
(25, 65.790)
(26, 62.730)
(27, 60.660)
(28, 63.490)
(29, 64.220)
(30, 63.390)
(31, 63.170)
(32, 62.610)
(33, 64.880)
(34, 65.240)
(35, 62.480)
(36, 64.010)
(37, 64.810)
(38, 65.620)
(39, 64.250)
(40, 65.830)
(41, 65.520)
(42, 66.260)
(43, 68.570)
(44, 68.080)
(45, 68.900)
(46, 68.710)
(47, 68.930)
(48, 69.340)
(49, 69.440)
(50, 69.770)
(51, 69.630)
(52, 69.430)
(53, 69.990)
(54, 69.390)
(55, 69.830)
(56, 69.400)
(57, 69.500)
(58, 69.340)
(59, 69.650)
};

==> figures/data/dfr-error-min.tex <==
\addplot[violet, densely dashed]
coordinates { % Fine-tune
(0, 37.210)
(1, 36.730)
(2, 37.230)
(3, 37.470)
(4, 37.340)
(5, 37.430)
(6, 35.960)
(7, 36.770)
(8, 37.780)
(9, 37.850)
(10, 38.070)
(11, 36.900)
(12, 38.530)
(13, 36.570)
(14, 37.690)
(15, 38.060)
(16, 38.270)
(17, 37.970)
(18, 37.930)
(19, 38.370)
(20, 38.590)
(21, 37.510)
(22, 38.850)
(23, 38.430)
(24, 37.200)
(25, 37.730)
(26, 38.300)
(27, 38.730)
(28, 38.340)
(29, 37.790)
(30, 39.110)
(31, 38.050)
(32, 38.280)
(33, 38.710)
(34, 38.460)
(35, 38.240)
(36, 39.050)
(37, 38.480)
(38, 39.380)
(39, 38.590)
(40, 39.200)
(41, 39.210)
(42, 39.550)
(43, 39.560)
(44, 39.170)
(45, 38.890)
(46, 39.310)
(47, 38.430)
(48, 39.000)
(49, 38.780)
(50, 39.160)
(51, 39.040)
(52, 39.070)
(53, 39.090)
(54, 39.420)
(55, 39.230)
(56, 39.080)
(57, 38.910)
(58, 38.110)
(59, 38.320)
};

==> figures/data/dfr-l2-ar.tex <==
\addplot[violet, densely dashed]
coordinates { % Fine-tune
(0, 39.210)
(1, 47.500)
(2, 55.260)
(3, 58.730)
(4, 47.770)
(5, 43.900)
(6, 40.130)
(7, 39.430)
(8, 38.820)
(9, 35.860)
(10, 34.970)
(11, 34.930)
(12, 33.460)
(13, 33.880)
(14, 35.530)
(15, 36.230)
(16, 29.470)
(17, 32.060)
(18, 31.280)
(19, 29.880)
(20, 30.880)
(21, 34.130)
(22, 28.460)
(23, 26.870)
(24, 30.210)
(25, 31.680)
(26, 27.770)
(27, 27.180)
(28, 32.600)
(29, 28.590)
(30, 30.300)
(31, 28.670)
(32, 29.520)
(33, 28.740)
(34, 27.990)
(35, 28.040)
(36, 30.950)
(37, 28.260)
(38, 29.200)
(39, 28.690)
(40, 29.220)
(41, 27.960)
(42, 29.030)
(43, 28.270)
(44, 29.040)
(45, 27.670)
(46, 30.000)
(47, 27.040)
(48, 27.160)
(49, 26.410)
(50, 27.720)
(51, 28.630)
(52, 27.460)
(53, 26.630)
(54, 27.790)
(55, 28.820)
(56, 28.680)
(57, 27.970)
(58, 27.930)
(59, 27.840)
};

==> figures/data/dfr-lsp.tex <==
\addplot[violet, densely dashed]
coordinates { % Test Acc
(0, 37.570)
(1, 37.860)
(2, 39.710)
(3, 41.120)
(4, 39.560)
(5, 39.450)
(6, 38.870)
(7, 38.850)
(8, 38.970)
(9, 38.790)
(10, 37.860)
(11, 36.420)
(12, 39.970)
(13, 34.390)
(14, 35.920)
(15, 36.670)
(16, 35.170)
(17, 35.300)
(18, 34.910)
(19, 32.330)
(20, 37.540)
(21, 34.080)
(22, 32.610)
(23, 31.090)
(24, 33.690)
(25, 34.550)
(26, 32.440)
(27, 31.900)
(28, 32.050)
(29, 29.300)
(30, 27.430)
(31, 32.270)
(32, 31.660)
(33, 31.810)
(34, 30.200)
(35, 29.680)
(36, 30.240)
(37, 33.510)
(38, 29.470)
(39, 27.950)
(40, 32.350)
(41, 33.140)
(42, 30.300)
(43, 29.360)
(44, 31.960)
(45, 31.490)
(46, 31.320)
(47, 30.890)
(48, 31.500)
(49, 31.310)
(50, 30.000)
(51, 31.000)
(52, 31.140)
(53, 31.920)
(54, 31.780)
(55, 32.310)
(56, 34.460)
(57, 33.660)
(58, 33.920)
(59, 32.450)
};

==> figures/data/dfr-ntga.tex <==
\addplot[violet, densely dashed]
coordinates { % Test Acc
(0, 37.670)
(1, 43.800)
(2, 49.090)
(3, 49.480)
(4, 49.750)
(5, 51.340)
(6, 49.310)
(7, 50.220)
(8, 48.660)
(9, 49.820)
(10, 52.810)
(11, 49.580)
(12, 51.470)
(13, 53.080)
(14, 51.590)
(15, 52.600)
(16, 50.770)
(17, 52.110)
(18, 52.940)
(19, 52.910)
(20, 51.220)
(21, 52.080)
(22, 50.810)
(23, 51.120)
(24, 50.850)
(25, 52.110)
(26, 52.570)
(27, 53.190)
(28, 53.170)
(29, 52.560)
(30, 52.710)
(31, 53.810)
(32, 53.030)
(33, 54.900)
(34, 51.110)
(35, 51.250)
(36, 55.090)
(37, 51.880)
(38, 56.160)
(39, 52.680)
(40, 54.380)
(41, 54.250)
(42, 53.800)
(43, 55.470)
(44, 55.600)
(45, 55.490)
(46, 56.450)
(47, 56.610)
(48, 56.700)
(49, 56.680)
(50, 56.090)
(51, 56.600)
(52, 56.510)
(53, 56.670)
(54, 56.740)
(55, 56.260)
(56, 57.000)
(57, 57.120)
(58, 56.760)
(59, 56.680)
};

==> figures/data/dfr-ops-plus-em.tex <==
\addplot[violet, densely dashed]
coordinates { % Test Acc
(0, 33.690)
(1, 33.630)
(2, 34.350)
(3, 32.250)
(4, 32.950)
(5, 33.850)
(6, 34.470)
(7, 34.420)
(8, 35.780)
(9, 33.610)
(10, 33.400)
(11, 32.160)
(12, 34.320)
(13, 32.470)
(14, 33.020)
(15, 35.410)
(16, 33.120)
(17, 32.080)
(18, 33.290)
(19, 28.740)
(20, 29.840)
(21, 31.910)
(22, 29.660)
(23, 31.010)
(24, 30.920)
(25, 29.570)
(26, 30.350)
(27, 29.800)
(28, 30.490)
(29, 29.100)
(30, 28.730)
(31, 28.060)
(32, 28.390)
(33, 28.680)
(34, 28.360)
(35, 28.240)
(36, 27.370)
(37, 31.120)
(38, 29.030)
(39, 29.490)
(40, 29.290)
(41, 29.380)
(42, 28.450)
(43, 30.170)
(44, 28.970)
(45, 28.880)
(46, 28.820)
(47, 28.680)
(48, 30.350)
(49, 30.300)
(50, 28.870)
(51, 29.160)
(52, 30.490)
(53, 29.130)
(54, 24.340)
(55, 26.760)
(56, 29.430)
(57, 21.480)
(58, 29.410)
(59, 28.470)
};

==> figures/data/dfr-ops.tex <==
\addplot[violet, densely dashed]
coordinates { % Test Acc
(0, 43.440)
(1, 38.850)
(2, 37.300)
(3, 39.300)
(4, 40.370)
(5, 35.270)
(6, 40.590)
(7, 34.490)
(8, 33.210)
(9, 34.220)
(10, 31.480)
(11, 31.120)
(12, 27.210)
(13, 25.030)
(14, 29.480)
(15, 24.660)
(16, 21.070)
(17, 28.980)
(18, 25.730)
(19, 24.850)
(20, 23.120)
(21, 25.150)
(22, 23.430)
(23, 24.580)
(24, 26.650)
(25, 26.040)
(26, 25.870)
(27, 27.870)
(28, 26.890)
(29, 27.260)
(30, 21.540)
(31, 27.380)
(32, 27.260)
(33, 27.400)
(34, 28.940)
(35, 27.160)
(36, 30.980)
(37, 24.640)
(38, 28.530)
(39, 23.710)
(40, 28.830)
(41, 28.250)
(42, 29.130)
(43, 27.110)
(44, 28.640)
(45, 27.270)
(46, 31.310)
(47, 31.840)
(48, 31.650)
(49, 30.620)
(50, 31.410)
(51, 31.730)
(52, 30.230)
(53, 31.600)
(54, 32.120)
(55, 30.640)
(56, 31.440)
(57, 31.510)
(58, 33.470)
(59, 32.100)
};

==> figures/data/dfr-regions-4.tex <==
\addplot[violet, densely dashed]
coordinates { % Test Acc
(0, 42.030)
(1, 43.530)
(2, 45.900)
(3, 46.340)
(4, 44.380)
(5, 47.140)
(6, 47.150)
(7, 46.640)
(8, 47.460)
(9, 48.090)
(10, 45.570)
(11, 45.380)
(12, 46.900)
(13, 45.810)
(14, 47.910)
(15, 46.000)
(16, 46.940)
(17, 46.480)
(18, 47.280)
(19, 45.340)
(20, 45.240)
(21, 43.660)
(22, 46.750)
(23, 44.350)
(24, 43.240)
(25, 44.570)
(26, 43.360)
(27, 43.020)
(28, 44.160)
(29, 44.040)
(30, 42.770)
(31, 43.110)
(32, 42.420)
(33, 44.080)
(34, 44.300)
(35, 42.040)
(36, 42.840)
(37, 44.220)
(38, 44.220)
(39, 43.560)
(40, 43.730)
(41, 44.770)
(42, 45.140)
(43, 45.090)
(44, 44.650)
(45, 45.560)
(46, 44.730)
(47, 43.850)
(48, 45.580)
(49, 45.250)
(50, 45.000)
(51, 44.910)
(52, 45.180)
(53, 44.910)
(54, 45.380)
(55, 45.160)
(56, 45.240)
(57, 45.220)
(58, 45.250)
(59, 45.510)
};

==> figures/data/dfr-robust-error-min.tex <==
\addplot[violet, densely dashed]
coordinates { % Test Acc
(0, 39.730)
(1, 36.070)
(2, 36.350)
(3, 37.270)
(4, 39.350)
(5, 36.570)
(6, 35.340)
(7, 38.880)
(8, 38.310)
(9, 37.950)
(10, 38.410)
(11, 37.180)
(12, 36.630)
(13, 38.960)
(14, 35.270)
(15, 37.730)
(16, 37.060)
(17, 38.040)
(18, 38.130)
(19, 41.020)
(20, 40.660)
(21, 36.520)
(22, 39.520)
(23, 39.280)
(24, 39.690)
(25, 39.940)
(26, 37.100)
(27, 38.040)
(28, 38.320)
(29, 38.510)
(30, 37.060)
(31, 37.440)
(32, 35.930)
(33, 36.030)
(34, 38.860)
(35, 39.110)
(36, 39.860)
(37, 38.660)
(38, 37.970)
(39, 37.840)
(40, 37.450)
(41, 39.990)
(42, 36.560)
(43, 38.650)
(44, 37.910)
(45, 39.000)
(46, 38.710)
(47, 38.710)
(48, 38.070)
(49, 37.860)
(50, 38.910)
(51, 39.090)
(52, 38.430)
(53, 38.870)
(54, 39.060)
(55, 38.960)
(56, 38.680)
(57, 38.830)
(58, 38.570)
(59, 39.050)
};

==> figures/data/error-max.tex <==
\addplot[violet]
coordinates { % Test Acc
(0, 46.350)
(1, 51.390)
(2, 24.890)
(3, 14.950)
(4, 15.190)
(5, 13.070)
(6, 10.420)
(7, 9.160)
(8, 9.970)
(9, 7.340)
(10, 7.880)
(11, 10.310)
(12, 7.500)
(13, 11.480)
(14, 13.330)
(15, 6.770)
(16, 7.580)
(17, 8.070)
(18, 8.740)
(19, 9.240)
(20, 8.510)
(21, 7.830)
(22, 6.690)
(23, 9.700)
(24, 8.980)
(25, 6.270)
(26, 7.280)
(27, 8.700)
(28, 9.340)
(29, 8.000)
(30, 9.550)
(31, 9.870)
(32, 9.340)
(33, 7.570)
(34, 7.880)
(35, 10.830)
(36, 5.740)
(37, 6.600)
(38, 7.520)
(39, 7.650)
(40, 9.310)
(41, 9.570)
(42, 8.760)
(43, 6.180)
(44, 7.270)
(45, 6.980)
(46, 7.180)
(47, 7.890)
(48, 7.500)
(49, 7.000)
(50, 6.980)
(51, 6.900)
(52, 6.910)
(53, 6.960)
(54, 6.980)
(55, 7.260)
(56, 6.980)
(57, 7.400)
(58, 7.470)
(59, 7.340)
};
    


==> figures/data/error-min.tex <==
\addplot[violet]
coordinates { % Test Acc
(0, 24.610)
(1, 23.230)
(2, 20.560)
(3, 20.860)
(4, 20.350)
(5, 22.130)
(6, 21.360)
(7, 21.070)
(8, 25.080)
(9, 24.720)
(10, 24.840)
(11, 22.690)
(12, 22.300)
(13, 21.990)
(14, 23.790)
(15, 23.020)
(16, 22.730)
(17, 23.930)
(18, 21.570)
(19, 20.720)
(20, 21.890)
(21, 21.900)
(22, 23.160)
(23, 20.960)
(24, 21.340)
(25, 24.870)
(26, 22.110)
(27, 24.260)
(28, 23.510)
(29, 21.950)
(30, 23.950)
(31, 22.080)
(32, 24.130)
(33, 22.340)
(34, 24.990)
(35, 22.050)
(36, 24.020)
(37, 22.510)
(38, 24.460)
(39, 22.430)
(40, 22.330)
(41, 23.100)
(42, 24.110)
(43, 24.090)
(44, 23.370)
(45, 23.250)
(46, 25.600)
(47, 24.640)
(48, 25.020)
(49, 24.860)
(50, 25.000)
(51, 24.700)
(52, 24.620)
(53, 24.460)
(54, 24.850)
(55, 24.870)
(56, 24.370)
(57, 24.250)
(58, 24.110)
(59, 24.250)
};
    


==> figures/data/l2-ar.tex <==
\addplot[violet]
coordinates { % Test Acc
(0, 36.340)
(1, 45.350)
(2, 53.830)
(3, 46.370)
(4, 19.450)
(5, 12.200)
(6, 10.610)
(7, 10.470)
(8, 10.200)
(9, 10.310)
(10, 12.250)
(11, 11.960)
(12, 10.090)
(13, 10.430)
(14, 10.030)
(15, 10.150)
(16, 10.130)
(17, 10.010)
(18, 10.000)
(19, 10.190)
(20, 12.020)
(21, 12.940)
(22, 10.040)
(23, 10.060)
(24, 10.670)
(25, 10.010)
(26, 10.060)
(27, 10.960)
(28, 10.050)
(29, 10.240)
(30, 10.920)
(31, 10.380)
(32, 10.230)
(33, 10.180)
(34, 10.070)
(35, 10.720)
(36, 10.150)
(37, 10.000)
(38, 10.090)
(39, 10.160)
(40, 10.140)
(41, 10.050)
(42, 10.320)
(43, 10.340)
(44, 10.040)
(45, 10.130)
(46, 10.460)
(47, 10.370)
(48, 10.460)
(49, 10.570)
(50, 10.340)
(51, 10.240)
(52, 10.300)
(53, 10.420)
(54, 10.390)
(55, 10.190)
(56, 10.290)
(57, 10.210)
(58, 10.410)
(59, 10.440)
};

==> figures/data/lsp.tex <==
\addplot[violet]
coordinates { % Test Acc
(0, 28.320)
(1, 24.070)
(2, 28.300)
(3, 24.670)
(4, 28.760)
(5, 23.920)
(6, 24.630)
(7, 23.910)
(8, 25.460)
(9, 25.030)
(10, 28.330)
(11, 25.620)
(12, 24.910)
(13, 22.000)
(14, 23.560)
(15, 26.220)
(16, 21.000)
(17, 23.180)
(18, 27.970)
(19, 23.690)
(20, 22.450)
(21, 24.580)
(22, 20.390)
(23, 20.330)
(24, 25.910)
(25, 23.760)
(26, 22.440)
(27, 24.030)
(28, 23.360)
(29, 21.360)
(30, 24.100)
(31, 24.740)
(32, 26.750)
(33, 31.510)
(34, 25.540)
(35, 26.320)
(36, 24.600)
(37, 28.480)
(38, 25.400)
(39, 24.630)
(40, 27.650)
(41, 28.860)
(42, 27.630)
(43, 24.380)
(44, 26.950)
(45, 28.460)
(46, 28.200)
(47, 26.480)
(48, 26.100)
(49, 26.150)
(50, 26.500)
(51, 27.170)
(52, 26.500)
(53, 26.350)
(54, 27.170)
(55, 26.470)
(56, 27.150)
(57, 27.220)
(58, 26.950)
(59, 27.140)
};

==> figures/data/ntga.tex <==
\addplot[violet]
coordinates { % Test Acc
(0, 30.750)
(1, 29.740)
(2, 31.610)
(3, 34.970)
(4, 32.200)
(5, 30.950)
(6, 31.240)
(7, 31.960)
(8, 28.710)
(9, 28.780)
(10, 34.290)
(11, 31.670)
(12, 33.030)
(13, 36.140)
(14, 31.660)
(15, 32.140)
(16, 33.280)
(17, 32.820)
(18, 34.340)
(19, 33.450)
(20, 33.410)
(21, 33.480)
(22, 29.080)
(23, 32.350)
(24, 32.480)
(25, 29.650)
(26, 32.980)
(27, 35.180)
(28, 37.610)
(29, 32.590)
(30, 33.960)
(31, 33.580)
(32, 35.470)
(33, 38.100)
(34, 33.660)
(35, 34.480)
(36, 37.100)
(37, 32.100)
(38, 42.400)
(39, 36.320)
(40, 37.970)
(41, 37.810)
(42, 36.830)
(43, 39.990)
(44, 39.780)
(45, 40.690)
(46, 41.870)
(47, 42.850)
(48, 42.400)
(49, 42.460)
(50, 42.300)
(51, 42.370)
(52, 42.820)
(53, 43.040)
(54, 43.130)
(55, 43.710)
(56, 43.300)
(57, 43.470)
(58, 43.540)
(59, 43.540)
};
    


==> figures/data/ops-plus-em.tex <==
\addplot[violet]
coordinates { % Test Acc
(0, 21.580)
(1, 19.600)
(2, 22.740)
(3, 19.160)
(4, 21.090)
(5, 21.850)
(6, 25.310)
(7, 22.810)
(8, 20.700)
(9, 23.800)
(10, 22.580)
(11, 22.260)
(12, 21.810)
(13, 21.670)
(14, 23.500)
(15, 24.090)
(16, 22.320)
(17, 20.140)
(18, 22.840)
(19, 18.680)
(20, 20.300)
(21, 22.310)
(22, 20.980)
(23, 19.420)
(24, 20.660)
(25, 18.750)
(26, 18.080)
(27, 18.950)
(28, 17.510)
(29, 18.920)
(30, 17.530)
(31, 15.370)
(32, 21.460)
(33, 15.980)
(34, 17.650)
(35, 20.590)
(36, 16.740)
(37, 18.260)
(38, 19.720)
(39, 21.030)
(40, 20.570)
(41, 16.880)
(42, 18.090)
(43, 19.370)
(44, 18.530)
(45, 18.390)
(46, 19.270)
(47, 19.050)
(48, 18.830)
(49, 19.070)
(50, 18.920)
(51, 19.030)
(52, 18.610)
(53, 19.110)
(54, 18.750)
(55, 19.520)
(56, 18.960)
(57, 18.970)
(58, 19.530)
(59, 18.760)
};

==> figures/data/ops.tex <==
\addplot[violet]
coordinates { % Test Acc
(0, 41.180)
(1, 22.670)
(2, 14.930)
(3, 28.800)
(4, 21.010)
(5, 14.550)
(6, 24.250)
(7, 17.450)
(8, 19.280)
(9, 11.660)
(10, 23.510)
(11, 20.570)
(12, 14.280)
(13, 11.860)
(14, 18.870)
(15, 12.410)
(16, 10.940)
(17, 14.930)
(18, 10.910)
(19, 12.960)
(20, 13.830)
(21, 16.390)
(22, 10.710)
(23, 13.950)
(24, 16.250)
(25, 13.460)
(26, 17.870)
(27, 9.350)
(28, 9.820)
(29, 16.340)
(30, 10.560)
(31, 12.950)
(32, 12.660)
(33, 9.120)
(34, 17.540)
(35, 12.380)
(36, 13.250)
(37, 13.260)
(38, 11.120)
(39, 13.870)
(40, 10.750)
(41, 18.950)
(42, 16.930)
(43, 17.290)
(44, 17.690)
(45, 11.880)
(46, 17.590)
(47, 14.360)
(48, 18.420)
(49, 18.860)
(50, 17.740)
(51, 16.960)
(52, 15.090)
(53, 17.730)
(54, 17.360)
(55, 18.310)
(56, 16.040)
(57, 16.830)
(58, 17.140)
(59, 17.270)
};

==> figures/data/random-init-network.tex <==
\addplot[red, loosely dotted]
coordinates { 
(0, 35.97)
(59, 35.97)
};

==> figures/data/regions-4.tex <==
\addplot[violet]
coordinates { % Test Acc
(0, 21.290)
(1, 22.980)
(2, 19.530)
(3, 17.950)
(4, 15.950)
(5, 19.910)
(6, 16.700)
(7, 16.420)
(8, 16.710)
(9, 17.620)
(10, 17.920)
(11, 15.540)
(12, 15.190)
(13, 15.880)
(14, 13.180)
(15, 15.400)
(16, 16.950)
(17, 14.000)
(18, 19.010)
(19, 13.680)
(20, 11.410)
(21, 11.270)
(22, 10.840)
(23, 11.950)
(24, 11.810)
(25, 10.640)
(26, 11.660)
(27, 10.670)
(28, 11.000)
(29, 10.420)
(30, 10.770)
(31, 10.090)
(32, 11.700)
(33, 10.510)
(34, 10.300)
(35, 10.420)
(36, 10.720)
(37, 10.530)
(38, 11.340)
(39, 10.250)
(40, 10.250)
(41, 10.360)
(42, 10.580)
(43, 10.160)
(44, 10.230)
(45, 10.170)
(46, 10.200)
(47, 10.120)
(48, 10.100)
(49, 10.100)
(50, 10.200)
(51, 10.160)
(52, 10.130)
(53, 10.150)
(54, 10.150)
(55, 10.150)
(56, 10.110)
(57, 10.160)
(58, 10.100)
(59, 10.110)
};

==> figures/data/robust-error-min.tex <==
\addplot[violet]
coordinates { % Test Acc
(0, 34.940)
(1, 20.230)
(2, 19.430)
(3, 23.520)
(4, 24.330)
(5, 15.570)
(6, 19.610)
(7, 23.750)
(8, 19.920)
(9, 18.730)
(10, 22.830)
(11, 22.960)
(12, 13.290)
(13, 20.610)
(14, 15.500)
(15, 21.990)
(16, 15.270)
(17, 21.840)
(18, 18.140)
(19, 24.300)
(20, 22.240)
(21, 16.340)
(22, 21.290)
(23, 20.960)
(24, 19.620)
(25, 23.530)
(26, 21.540)
(27, 18.980)
(28, 24.010)
(29, 17.860)
(30, 14.230)
(31, 22.210)
(32, 19.290)
(33, 15.640)
(34, 19.470)
(35, 21.910)
(36, 20.770)
(37, 23.940)
(38, 21.010)
(39, 24.540)
(40, 22.090)
(41, 25.720)
(42, 24.320)
(43, 24.500)
(44, 22.210)
(45, 24.660)
(46, 20.890)
(47, 27.620)
(48, 24.630)
(49, 23.100)
(50, 26.840)
(51, 25.820)
(52, 26.120)
(53, 26.900)
(54, 26.270)
(55, 25.910)
(56, 26.230)
(57, 25.540)
(58, 26.290)
(59, 25.650)
};
